Pop-up SLAM: Semantic Monocular Plane SLAM for Low-texture Environments

Existing simultaneous localization and mapping (SLAM) algorithms are not robust in challenging low-texture environments because there are only few salient features. The resulting sparse or semi-dense map also conveys little information for motion planning. Though some work utilize plane or scene layout for dense map regularization, they require decent state estimation from other sources. In this paper, we propose real-time monocular plane SLAM to demonstrate that scene understanding could improve both state estimation and dense mapping especially in low-texture environments. The plane measurements come from a pop-up 3D plane model applied to each single image. We also combine planes with point based SLAM to improve robustness. On a public TUM dataset, our algorithm generates a dense semantic 3D model with pixel depth error of 6.2 cm while existing SLAM algorithms fail. On a 60 m long dataset with loops, our method creates a much better 3D model with state estimation error of 0.67%.

==> analysis.tex <==
In this section, we discuss some details of plane SLAM.





\subsection{Height effects}

Unlike the RGB-D plane SLAM, our plane measurement comes from the pop-up plane whose scale is determined by the camera height in Section \ref{sec:pop_up_pose}. So the SLAM plane measurements themselves cannot constraint the camera height anymore, which can only be constrained by other information such as odometry measurements or other sensors such as IMU. If these information is not accessible, the map scale will drift using the plane SLAM alone.

During all the experiments, we didn't meet the scale drifting problem because the cameras are kept at nearly constant height. If 

During all the experiments, we assume that cameras are kept at nearly a constant height so that our algorithm can keep the global scale.

During the experiments, we assume that the initial camera height to be 1m or using ground truth height in order to get an absolute 3D plane model scale. 

The cameras are kept at nearly a constant height in all the experiments performed above, our algorithm can keep the global scale without drifting.

But if this assumption is violated or relaxed, our \textit{Pop-up plane SLAM} might not keep scale consistency.

%But if this assumption is violated or relaxed, our \textit{Pop-up plane SLAM} might not keep scale consistency.

%During the experiments, we assume that the initial camera height to be 1m or using ground truth height in order to get an absolute 3D plane model scale. 
%The cameras are kept at nearly a constant height in all the experiments performed above, our algorithm can keep the global scale without drifting.





\subsection{sparsification}


\subsection{Limitations and future work}

